Reinforcement Learning-Based Dynamic Management of Structured Parallel Farm Skeletons on Serverless Platforms

We present a framework for dynamic management of structured parallel processing skeletons on serverless platforms. Our goal is to bring HPC-like performance and resilience to serverless and continuum environments while preserving the programmability benefits of skeletons. As a first step, we focus on the well known Farm pattern and its implementation on the open-source OpenFaaS platform, treating autoscaling of the worker pool as a QoS-aware resource management problem. The framework couples a reusable farm template with a Gymnasium-based monitoring and control layer that exposes queue, timing, and QoS metrics to both reactive and learning-based controllers. We investigate the effectiveness of AI-driven dynamic scaling for managing the farm's degree of parallelism via the scalability of serverless functions on OpenFaaS. In particular, we discuss the autoscaling model and its training, and evaluate two reinforcement learning (RL) policies against a baseline of reactive management derived from a simple farm performance model. Our results show that AI-based management can better accommodate platform-specific limitations than purely model-based performance steering, improving QoS while maintaining efficient resource usage and stable scaling behaviour.

==> notesReactiveFarm.tex <==
We defined and implemented a simple reactive policy \texttt{ReactiveAverage} that aims at the ideal parallelism degree provided by the basic farm performance model for the FastFlow-like farm template%\cite{danelutto2014structured}
~\cite{aldinucci2017guide}  described in the main work. At steady state, assuming the emitter and collector are no bottleneck (which we can verify in Fig.~\ref{fig:scaling_metrics} for $p\in [1,32]$), the optimal farm parallelism becomes $p = T_s / T_\textit{par}$, where $T_\textit{par}$ is the parallel service time we aim at and $T_s = \bar{T}_\textit{proc}$ is the moving average of task service time. For each \emph{step} interval of duration $T_\textit{step}$, our reactive policy attempts to compute the ideal steady-state parallelism that would be needed to keep up with the current load. It thus evaluates three components of parallelism:
\begin{itemize}
    \item 
for $k$ new tasks arriving during the interval, we require $p$ workers,
$p= T_s/T_\textit{int} \quad \textrm{where} \quad T_\textit{int}=T_\textit{step}/k$
    \item 
for $l$ leftover tasks in the worker queue since previous steps, we require 
$p'= T_s \, l / T_\textit{step}$ workers; we thus treat delayed tasks as if they arrived over the current step interval
    \item 
for a number $m$ of active tasks within the farm template, we require $p'' = T_s m / (2 T_\textit{step})$ more workers. As dynamic scaling deviates from steady state, we add this correction factor proportional to the amount of work in progress, assuming it is $T_s/2$ per task. This limits scale-down actions when the farm workers are busy ($m \gg 1$).
\end{itemize}

Overall, when $w$ is the current number of workers, the resource allocation change we perform is 
$$\Delta = p + p' - w +p'' = \frac{\bar{T}_\textit{proc}}{T_\textit{step}} (k+l+\frac{m}{2}) -w$$

The \texttt{ReactiveMaximum} policy is defined along the same lines, but it always chooses to overestimate the amount of work per task. Hence it uses the maximum observed processing time per step $T^\textit{max}_\textit{proc}$ in place of the average service time $T_s$, as well as for estimate of active tasks within the template.
The overall resource allocation change is thus computed as
$$\Delta_\textit{max} = \frac{T^\textit{max}_\textit{proc}}{T_\textit{step}} (k+l+m) -w $$
%\hrulefill\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% what follows is unused and incomplete
\begin{comment}
    
\todo{we may later summarize this, now I need to be quick.}
We defined and implemented a simple reactive policy assessing the ideal parallelism degree by employing the basic farm performance model. With parameters as outlined in Table\ref{tab:reactive_sym}, and farm implementation with emitter and collector processes (\emph{add reference}), the service time at steady state is
\[T_F = \frac{T_s}{p} \]
where we assume the emitter and collector are no bottleneck if parallelism does not exceed a given value $p_\textit{MAX}$. The optimal parallelism at steady state is 
\[p= \frac{T_s}{T_F}\ , \qquad 1 \leq p \leq p_\textit{MAX} \]
that we can compute in relation to the interarrival time as
$p= T_s/T_{int}$
%\emph{or to a specified QoS time constraint\footnote{this is a per-task parameter, TBD: how to generalize/summarize for a set of tasks}} \, $p= \alpha T_{QoS}$

We measure the interarrival time of tasks over a discrete time interval $T_{step}$, when we receive a batch of requests for that interval. By looking at the input queue $Q_W$ and its length $k$ at the beginning of the time interval we estimate the interarrival time as $T_{int}=T_{step}/k$ and compute the ideal parallelism  
\[p = \frac{T_s}{T_{step}}k\]
As we are predicting the behavior 
The simplest policy will compute $p$ and compare with current parallelism degree $p'$, then try to adapt by choosing the best available action $a \in \{-1, 0, +1\}$ i.e. the one minimizing $|p-(p'+a)|$.

As we are dealing with dynamic changes (changing interarrival time, $T_s$ as a stocastic variable) and correction actions are not immediate, the simple policy may not be able to ramp up parallelism quickly enough to scale up ideally, deviating from steady state behavior. One advantage of this policy is that previous tasks left unattended in the queue will sum to the new ones in the next interval, increasing our load metric (i.e. lower measured $T_\textit{int}$) and causing a stronger push for more parallelism (higher $p$).

\todo{in the works; maybe a simpler formulation can be done with two random vars for $T_s$ and $T_{QoS}$}

QoS definition and QoS-aware reactive policy. Each task $x$ will come with a QoS specification as a deadline $T_s(x)$ for service time that must be met, with constraint $T_\textit{QoS} > T_s$ . We want our policy to steer the farm to comply the deadline for all tasks, so we can initially replace our $T_s$ with $T_\textit{QoS}$, and compute parallelism from that: $p=k T_\textit{QoS}/T_\textit{step}$.


\todo{discuss case of leftover tasks; add Q  oS definition and integrate; what if we look at past interval metrics instead, is that simpler?}

\begin{table}[]
    \centering
    \begin{tabular}{ll}
    \toprule
       $p$  & degree of parallelism \\
       $T_s$  & average service time per task (sequential computation)\\
       $T_F$  & service time for the farm skeleton \\
       $T_\textit{int}$ & task interarrival time at farm input \\
       $T_\textit{QoS}$ & task service time as stipulated by QoS (TBD) \\
       $\alpha$ & constant multiple of the QoS deadline to target, $0 < \alpha < 1$ \\
    \midrule
    $T_{step}$ & duration of a discrete time step \\
    $Q_W$ & task queue feeding farm workers \\
    $q$ & length of $Q_W$ \\
    \bottomrule
    \end{tabular}\\[1ex]
    \caption{Symbols for the reactive policy based on the behavioral model of the farm}
    \label{tab:reactive_sym}
\end{table}

% USL Gunther 1993 related to Amdhal Law , look up bib here http://www.perfdynamics.com/Manifesto/USLscalability.html
\end{comment}

